Aligning Coordinated Text Streams through Burst Information Network Construction and Decipherment

Aligning coordinated text streams from multiple sources and multiple languages has opened many new research venues on cross-lingual knowledge discovery. In this paper we aim to advance state-of-the-art by: (1). extending coarse-grained topic-level knowledge mining to fine-grained information units such as entities and events; (2). following a novel Data-to-Network-to-Knowledge (D2N2K) paradigm to construct and utilize network structures to capture and propagate reliable evidence. We introduce a novel Burst Information Network (BINet) representation that can display the most important information and illustrate the connections among bursty entities, events and keywords in the corpus. We propose an effective approach to construct and decipher BINets, incorporating novel criteria based on multi-dimensional clues from pronunciation, translation, burst, neighbor and graph topological structure. The experimental results on Chinese and English coordinated text streams show that our approach can accurately decipher the nodes with high confidence in the BINets and that the algorithm can be efficiently run in parallel, which makes it possible to apply it to huge amounts of streaming data for never-ending language and information decipherment.

==> 1introduction__Ge_Tao____________2016-04-29_.tex <==
\section{Introduction}\label{sec:intro}

% low-resource situation. cross-lingual realistic, full-document MT is not realistic, but it's still useful to translate information networks...


In this information era, a large amount of text data is continuously produced over time in various applications (e.g., news agencies and social networks), which results in massive streams of text data with much valuable information and knowledge. Streaming data is an important source for many applications such as disaster summarization~\cite{Kedzie2015}.
There are many studies on pattern mining from text data streams but most of them focus on a single text stream. Nonetheless, there are many text streams that are topically related and indexed by the same
set of time points, which are called \emph{coordinated text streams}~\cite{Wang2007}. For example, news streams from a news agency in different languages are coordinated. In recent, text mining on coordinated text streams has gained attention in both data mining and natural language processing communities because one can discovery useful facts and important patterns. %by mining from coordinated text streams. 
For example, \cite{Wang2007} and \cite{zheng2012cross} tried to discover common topic patterns from coordinated text streams. In this paper, we aim to advance state-of-the-art from the following two perspectives.

(1) \textbf{Aligning Fine-grained Information Units instead of Coarse-grained Topics}.


\begin{figure*}[t]
\centering
\includegraphics[width=11cm]{Figures/walkthrough.pdf}
\caption{(A small part of) Burst information networks constructed from Chinese and English. 
%Note that the information networks in the figure is just a small part of the whole information networks constructed from the comparable corpora used in this paper.
\label{fig:walkthrough}}
\end{figure*} 

Most documents in coordinated streams are not entirely parallel. Fortunately, topically related and temporally correlated important facts such as bursty events and entities often repeatedly co-occur across streams from different languages.  
%As claimed, coordinated streams usually contain. 
Most previous work on coordinated text stream mining such as~\cite{Wang2007} analyzed the streams on the coarse-grained topic level, which inevitably leads to loss of some information. For instance, a topic-level cross-lingual text stream analysis cannot inform us the mentions of an entity in the other text stream. For fully exploiting the coordinated text streams, we propose to analyze the text streams by attempting to align important fine-grained information units (e.g., entities and events) across the streams. Specifically, in this paper, we focus on aligning cross-lingual coordinated text streams. We choose two very different languages -- Chinese and English streams for alignment as a case study. Aligning cross-lingual coordinated text streams is a meaningful task because it can mine translation pairs for completing a bi-lingual lexicon, which would be helpful for cross-lingual information extraction, information retrieval and machine translation systems that suffer from bi-lingual lexicons with a limited number of entries. 


% make motivations and novel claims very clear
%In this paper, we advance state-of-the-art from the following three perspectives
%However, most previous work focused on topic-level alignment
%(1). extend coarse-grained topic-level knowledge mining to fine-grained information units such as entities and events; (2). follow a novel ``\emph{data-to-network-to-knowledge (D2N2K)'' paradigm to construct and utilize network structures to capture and propagate more reliable evidence. 

(2) \textbf{Data-to-Network-to-Knowledge (D2N2K) instead of Data-to-Knowledge (D2K)}
% add tutorial words... overwhelming. slow down the process
%Using a structured representation (e.g., graph, network) as a bridge to capture interactions between NLP and DM
% add inter-dependency. not independent. network structures... neighbors. topological structures, propagate... power of network

Instead of directly turning massive, unstructured data streams into structured knowledge (D2K), we propose a new Data-to-Network-to-Knowledge (D2N2K) paradigm, based on the following observations: (i) most information units are not independent, instead they are interconnected or interacting, forming massive networks; (ii) if  information networks can be constructed across multiple languages, they may bring tremendous power to make knowlege mining algorithms more scalable and effective because we can take advantage of the graph structures to acquire and propagate knowledge. For aligning the cross-lingual text streams, we first propose a novel text stream's structured representation called ``\emph{Bursty Information Networks (BINets)}'' to focus on the most important information units. In BINets, nodes are bursty words including important entities and events, and edges represent their co-burst relations. A word's burst refers to a remarkable increase in the number of occurrences of the word during a short period of time. An example is depicted in Figure~\ref{fig:walkthrough}. Similar to traditional Information Networks~\cite{Han2010,Li2014}, nodes within a community in BINets are semantically related (e.g., entities are often participants in certain events). Moreover, they are also temporally coherent. For example, the nodes in Figure~\ref{fig:walkthrough} are all related to the 2010 Australian Open.


%Bursts and time series are important information to conduct cross-lingual topic level analysis. \newcite{Wang2007} proposed to mine correlated bursty topic patterns from coordinated text stream using a probability mixture model. \newcite{wang2009mining} loosed the constraint of the coordinated stream; instead, they studied mining bursty topic pattern from asynchronous text stream.  \newcite{zheng2012cross} studied topic alignment in time series of Chinese/Japanese news.



%our goal:

% we target at information unit decipherment, a large scope. 
% to narrow down, we use burst event graph

% but we cannot check all possible candidate pairs.
% so we propose a novel method to construct burst event graph.


%but manual translations for these oov are not available, not complete.
%XXX still need to translate it, ...but many words are OOV... fortunately, ...burst information is usually shared across languages... 

After the BINets are constructed, our next goal is to align the nodes in BINets across text streams. In comparable corpora, bursty words which are about either a breaking news or a hot topic usually burst across languages. For example, both ``澳洲网球公开赛(Australian Open)'' and its translation in English ``Australian Open'' in figure \ref{fig:walkthrough} burst from Jan 14 to Jan 31 in 2010. We take advantage of such characteristics of bursts across languages and propose four decipherment clues from some starting points (prior knowledge) in a propagation manner. Experimental results demonstrate that our aligning approach can accurately mine cross-lingual translation pairs and that the more data provided, the more translation pairs will be discovered, which means that if our approach can run over the streaming data produced throughout the time, it will be a never-ending translation pair discovery framework.

% and it is promising to apply our approach to a large volume of comparable corpora for the acquition of translation of out-of-vocabulary words.

%The main novel contributions of this paper are as follows:
%\begin{itemize}
%\item For the first time we propose to model the translation pair mining from comparable corpora as a network decipherment problem.
%\item Based on the characteristics of co-burst across languages, we propose four novel and effective clues to decipher BINets.
%\end{itemize}





% % % % % % % % %COMMENTS % % % % % % % % % % % % %
%\todo{both title and section titles need to be refined. I'm struggling between knowledge networks and information networks}
%\todo{the figure is just a place holder, replace it with real examples, and change it to burst graph}

%Innovative Use of Domain-Rich, Non-Parallel Data: Found parallel data will be inadequate for creating domain-specific IL capabilities. We introduce new techniques, applied to both IE and topic processing capabilities, for projecting English and LRLP structural knowledge to IL, by inferring projections using domain-rich, non-parallel data. 

%Cross-lingual information projection and mining across non-parallel data. 
%We propose a major new research direction – the projection of IE across domain-rich, non-parallel corpora (e.g., coordinated news streams [Wang et al. 07], code-switching in social media [Voss et al. 14; Tratz et al. 14ab]).  Figure 3 illustrates our idea. 



==> 2.1burst__Ge_Tao____________2016-04-29_.tex <==
\subsection{Burst Detection}
%A word's burst refers to a remarkable increase in the number of occurrences of the word during a short period of time. 

To build a bursty information network mentioned in Section \ref{sec:intro}, we first need to detect bursts of words. In general, a word's burst might indicate  important events or trending topics. For example, the word ``威廉(Williams)'' has a burst from Jan 27 to Jan 31, as shown in Figure \ref{fig:bstate} because of the wonderful performance of Serena Williams in the 2010 Australian Open held during this period. For a timestamped document collection $\mathbf{C}=\{D_1,D_2,...,D_\tau,...,D_{T}\}$ where $D_\tau$ is the collection of documents during time $\tau$, we define a word $w$'s burst sequence $\boldsymbol{s}=(s_1,s_2,...,s_\tau,...,s_T)$ in which $s_\tau$ is either 1 or 0 to indicate if $w$ bursts or not at the time epoch. Based on the ideas from \cite{kleinberg2003bursty,zhao2012novel}, this burst sequence can be simply found by searching for the optimal sequence $\boldsymbol{s}^{*}$ to minimize the cost function defined as follows:

\begin{equation}\label{eq:burst}
\begin{split}
& Cost(\boldsymbol{s},\boldsymbol{p},q^{(0)},q^{(1)})= \\
& \sum_{t=1}^T|\log p_\tau-\log q^{(s_\tau)}| + \sum_{\tau=1}^{T-1}\beta*\mathbf{1}(s_\tau \neq s_{\tau+1})
\end{split}
\end{equation}
\noindent where $\boldsymbol{p}=(p_1,...,p_\tau,...,p_T)$ in which $p_\tau$ is the probability of the word at $\tau$, $q^{(0)}$ is the base probability of the word and it is often defined as the probability of the word on the whole data/corpus, $q^{(1)}$ is the burst probability of the word and it is often defined as $q^{(1)}=\alpha q^{(0)}$ ($\alpha>1$). 

The first term of Eq (\ref{eq:burst}) measures the difference between $p_\tau$ and $q^{(s_\tau)}$. If a word bursts (i.e., $p_\tau$ is high), $s_\tau=$1 will yield less cost and thus in the optimal sequence $\boldsymbol{s}^{*}$, $s_\tau$ tends to be 1; otherwise, $s_\tau$ tends to be 0. The last term of Eq (\ref{eq:burst}) is for penalizing transition of burst states through the time to avoid too frequent transition of burst states for smoothing and $\beta$ is the parameter controlling this part's weight\footnote{In our experiments, we empirically set $\alpha=9$, $\beta=1$.}.

\begin{figure}[t]
\centering
\includegraphics[width=8.5cm]{Figures/ambiguity.pdf}
\caption{Burst state of ``威廉(Williams)'' during 2010. The horizontal axis is time (days after Jan 1, 2010) and the vertical axis is the burst state of the word, which is either 1 or 0 to indicate if the word bursts or not. The first two bursts refer to Serena Williams while the last two bursts refer to Prince Williams.\label{fig:bstate}}
\end{figure}

Specifically, if a word $w$ bursts at every time $\tau$ during a period, we call this period as a burst period of $w$, and $w$ has a burst during this period. In Figure \ref{fig:bstate}, we can see that the word ``威廉(Williams)'' has 4 burst periods. %so we say ``威廉(Williams)'' has 4 bursts. 
Formally, we define $\mathcal{P}_w$ as one of burst periods of the word $w$. $\mathcal{P}_w$ is a consecutive time sequence during which $w$ bursts at every time epoch $\tau$:

\centerline{
$\mathcal{P}_w=(\tau_i,\tau_{i+1},\tau_{i+2},...,\tau_{i+n})$
}
\centerline{
$\forall \tau \in \mathcal{P}~~s_\tau(w)=1$
}
\noindent where $s_\tau(w)$ denotes the burst state of $w$ at time $\tau$.

==> 2.1burst__Heng_Ji_s_conflicted_copy_2015-12-22_.tex <==
\subsection{Burst Detection}
%A word's burst refers to a remarkable increase in the number of occurrences of the word during a short period of time. 
\begin{figure*}[t]
\centering
\includegraphics[width=14cm]{Figures/ambiguity.pdf}
\caption{Burst state of ``威廉(Williams)'' during 2010. The horizontal axis is time (days after Jan 1, 2010) and the vertical axis is the burst state of the word, which is either 1 or 0 to indicate if the word bursts or not. The first two bursts refer to Serena Williams while the last two bursts refer to Prince Williams.\label{fig:bstate}}
\end{figure*}

To build a bursty information network mentioned in Section \ref{sec:intro}, we first need to detect bursts of words. In general, a word's burst might indicate  important events or trending topics. For example, the word ``威廉(Williams)'' has a burst from Jan 27 to Jan 31, as shown in Figure \ref{fig:bstate} because of the wonderful performance of Serena Williams in the 2010 Australian Open held during this period. For a timestamped document collection $\mathbf{C}=\{D_1,D_2,...,D_\tau,...,D_{T}\}$ where $D_\tau$ is the collection of documents during time $\tau$, we define a word $w$'s burst sequence $\boldsymbol{s_w}=(s_1,s_2,...,s_\tau,...,s_T)$ in which each entry is either 1 or 0 to indicate if $w$ bursts or not at the time epoch. Based on the ideas from \cite{kleinberg2003bursty,zhao2012novel}, this burst sequence can be simply found by searching for the optimal sequence $\boldsymbol{s}^{*}$ to minimize the cost function defined as follows:

\begin{equation}\label{eq:burst}
\small
Cost(\boldsymbol{s},\boldsymbol{p},q^{(0)},q^{(1)})=\sum_{t=1}^T|\log p_\tau-\log q^{(s_\tau)}| + \sum_{\tau=1}^{T-1}\beta*\mathbf{1}(s_\tau \neq s_{\tau+1})
\end{equation}
where $\boldsymbol{s}=(s_1,s_2,...,s_\tau,...,s_T)$ where $s_\tau$ denotes the burst state of the word at time $\tau$, $\boldsymbol{p}=(p_1,p_2,...,p_\tau,...,p_T)$ where $p_\tau$ is the probability of the word at $\tau$, $q^{(0)}$ is the base probability of the word and it is often defined as the probability of the word on the whole data/corpus, $q^{(1)}$ is the burst probability of the word and it is often defined as $q^{(1)}=\alpha q^{(0)}$ ($\alpha>1$), $\mathbf{1}(\cdot)$ is the indicator function, and $\beta$ is the parameter for controlling the weight of penalizing transition of burst states across the time\footnote{In our experiments, we empirically set $\alpha=9$, $\beta=1$}.

The first part of Eq (\ref{eq:burst}) measures the difference between $p_\tau$ and $q^{(s_\tau)}$. if a word bursts (i.e., $p_\tau$ is high), $|log p_\tau-log q^{(1)}|$ is smaller than $|log p_\tau-log q^{(0)}|$; otherwise, it is larger than $|log p_\tau-log q^{(0)}|$. The second part of Eq (\ref{eq:burst}) is for penalizing transition of burst states across the time for avoiding too frequent transition of burst states.

Specifically, if a word $w$ bursts at every time $\tau$ during a period, we call this period as a burst period of $w$, and $w$ has a burst during this period. In Figure \ref{fig:bstate}, we can see that the word ``威廉(Williams)'' has 4 burst periods. %so we say ``威廉(Williams)'' has 4 bursts. 
Formally, we define $\mathcal{P}_w$ as one of burst periods of the word $w$. $\mathcal{P}_w$ is a consecutive time sequence during which $w$ bursts at every time epoch $\tau$:
\begin{displaymath}
\mathcal{P}_w=(\tau_i,\tau_{i+1},\tau_{i+2},...,\tau_{i+n})
\end{displaymath}
\begin{displaymath}
\forall \tau \in \mathcal{P}~~s_\tau(w)=1
\end{displaymath}
where $s_\tau(u)$ denotes the burst state of $w$ at time $\tau$.

==> 2.3centroid.tex <==
\subsection{Centroid Detection}
In the bursty information network, there are a small portion of nodes that are centroid of a community. In general, these centroid nodes are influential and keywords of a topic.

In order to detect such centroid in the bursty information network, we use the Pagerank algorithm to randomly walk the bursty information network.

To do: briefly introduce the details of pagerank in this problem.

==> 4mining.tex <==
\section{Mining}

%XXX lots of bi-products
% by the way... can do xdoc coreference, can correct IE errors.

%Once the initial InfoNets are jointly constructed and translated, many powerful knowledge extraction mechanisms are enabled.  First, we propose to iteratively extract new name translation pairs. We start from common name translations or language-universal representations such as time/calendar date, number, website URL, currency and emoticons (e.g., “埃博拉-Ebola,” “39人-39 people, and “2014/11/25 – 2014/11/25” in Figure 2), and then obtain new pairs with a large portion of overlapped links.  For example, based on the assumption that if the same number of people died on the same date due to the same cause, then they are likely to share the same location, we can acquire the name pair of “科纳克里 – Conakry.” We will exploit additional novel constraints such as IPA similarity, name transliteration, temporal distributions, graph structure, topic and distributional similarity. We will also design novel graph-based alignment algorithms and rank link types based on discriminative power (e.g., links like ‘date-of-birth,’ ‘origin,’ and ‘religion’ are less informative than links like ‘website’ and ‘founded’).  In addition, we propose to cluster and rank nodes to detect influential roles and outliers across languages as emergent entities. Moreover, we will disambiguate entities, construct their profiles and predict hidden relations simultaneously during the alignment using Meta-Path [Huang et al. 13; Zhang et al. 14]. This self-boosting framework will mutually enhance extraction and translation acquisition, and demonstrate a successful joint inference procedure across disparate knowledge sources from multiple languages.

%\todo{talk about how to construct and update the cross-lingual matrix; need a better subtitle}
\subsection{New Word Translation Mining}
\subsection{Influential Role Mining}
\subsection{Outlier Mining}
\subsection{Cross-document Entity Coreference Resolution}



==> 5experiment__Heng_Ji_s_conflicted_copy_2015-12-22_.tex <==
\section{Experiments}
\begin{figure*}[!htb]
\centering
\includegraphics[width=13.5cm]{Figures/cluevalidation.pdf}
\caption{Accuracy curves of various approaches. Note that \textit{pv+tv+nv+cv} is our final approach\label{fig:topk}}
\end{figure*}
\input{5.1data}
\input{5.2setting}
\input{5.3results}


==> 6related__Heng_Ji_s_conflicted_copy_2015-12-22_.tex <==
\section{Related Work}

Burst patterns have been studied for decades in data mining and natural language processing communities. \cite{swan2000timemines,kleinberg2003bursty,zhao2012novel} studied burst detection problem from text streams. \cite{swan2000timemines,fung2005parameter,Wang2007,he2007using,diao2012finding,zhao2012novel} employed burst information to find bursty topics and events.

Extensive research has also been done on bilingual lexicon induction (e.g.,~\cite{Fung1998,Rapp1999,koehn2002learning,schafer2002inducing,Shao2004,schafer2006translation,Hassan2007,Haghighi2008,Udupa2009,Klementiev2010,Irvine2013}) and name translation mining (e.g.,~\cite{Sproat2006,klementiev2006weakly,ji2009mining,You2010,Lin2011}) from non-parallel corpora. Some of these approaches also exploited temporal similarity. We proposed new and richer clues including burst and graph topological structure. The nodes in BINet are not limited to named entities. More importantly, it is much cheaper to construct BINets than traditional information networks which usually rely on supervised information extraction or a large set of seed translation pairs.


%the projtion of IE
In contrast to previous cross-lingual projection work like data transfer~\cite{Pado2009} and model transfer~\cite{McDonald2011}, we do not require any parallel data. 
%burst word network...
% burst event paper didn't apply to cross-lingual
Our BINet construction method was inspired by~\cite{sayyadi2013graph}. Our work is the first to apply it to a cross-lingual setting. This is also the first attempt to apply the decipherment idea (e.g., \cite{Ravi2011,Dou2012,Dou2014}) to graph structures instead of sequence data. Another work related to ours is \cite{kotov2011mining} which uses correlated burst information to discover transliteration of entities, which is somewhat similar to $pv$ baseline. Compared with their work, this paper addresses a more general problem -- we not only focus on transliteration of named entities but all kinds of out-of-vocabulary words and phrases based on both similarities of pronunciation, translation, context and temporal correlation.

% % % % % % % % % % % % % % %COMMENTS % % % % % % % % % % % %

% the following from
%http://nlp.cs.rpi.edu/paper/NameMining.pdf
%
%Most  of  the  previous  name  translation  work  com-
%bined  supervised  transliteration  approaches  with
%Language Model based re-scoring (Al-Onaizan and
%Knight,  2002;  Huang  et  al.,  2004;  Huang,  2005).
%Our goal of addressing name translation for a large
%number of languages is similar to the panlingual lex-
%ical translation project (Etzioni et al., 2007).  Some
%recent research used comparable corpora to re-score
%name transliterations (Sproat et al., 2006; Klemen-
%tiev  and  Roth,  2006)  or  mine  new  word  transla-
%tions (Udupa et al., 2009;  Ji, 2009;  Fung and Yee,
%1998; Rapp, 1999; Shao and Ng, 2004; Hassan et al.,
%2007).  However, most of these approaches needed
%large  amount  of  seeds  and  suffered  from  informa-
%tion  extraction  errors,  and  thus  relied  on  phonetic
%similarity or document similarity to re-score candi-
%date name translation pairs
%
%
%Ji  et
%al.  (2009)  described  various  approaches  to  auto-
%matically mine name translation pairs from aligned
%phrases  (e.g.    cross-lingual  Wikipedia  title  links)
%or  aligned  sentences  (bi-texts).
%?
%)   mined  candi-
%date  words  from  Wikipedia  and  validated  transla-
%tions based on parallecl corpora.  Some other work
%mined  name  translations  from  mono-lingual  docu-
%ments that include foreign language texts. For exam-
%ple, Lin et al. (2008) described a parenthesis transla-
%tion mining method; You et al. (2010) applied graph
%alignment algorithm to obtain name translation pairs
%based  on  co-occurrence  statistics.     This  kind  of
%data does not commonly exist for low-density lan-
%guages. Sorg and Cimiano (2008) discovered cross-
%lingual links between English and German using su-
%pervised classification based on support vector ma-
%chines.  Adar et al. (2009) aligned cross-lingual in-
%foboxes  using  a  boolean  classifier  based  on  self-
%supervised training with various linguistic features.
%In contrast, our approach described in this paper is
%entirely based on unsupervised learning without us-
%ing  any  linguistic  features.   de  Melo  and  Weikum
%(2010) described an approach to detect imprecise or
%wrong cross-lingual Wikipedia links based on graph
%repair operations.   Our algorithm can help recover
%those missing cross-lingual links.

% And need to cite many cross-lingual word dictionary induction papers; refer to CCB's paper's related work

%We also propose to extend our discriminative model for bilingual lexicon induction [Irvine and Callison-Burch 13b]. The discriminative model allows us to combine multiple, monolingually estimated signals of translation equivalence (like contextual similarity, temporal similarity, orthographic similarity). We demonstrated that this model outperforms previous unsupervised approaches [Schafer and Yarowsky 02, Haghighi et al. 08]. We propose to improve the model by incorporating external knowledge in the form of high-resource languages that are related to the IL, structured linguistic information like the World Atlas of Language Structures Online [Dryer and Haspelmath 13], and the paraphrase database [Ganitkevitch et al. 13]. We will use human informants to improve training [Zaidan and Callison-Burch 09, Pavlick et al. 14]. 

% cite some work on X-do entity coreference resolution or NIL clustering work. use Zheng's collborative clustering paper's related work

%We also propose to extend our discriminative model for bilingual lexicon induction [Irvine and Callison-Burch 13b]. The discriminative model allows us to combine multiple, monolingually estimated signals of translation equivalence (like contextual similarity, temporal similarity, orthographic similarity). We demonstrated that this model outperforms previous unsupervised approaches [Schafer and Yarowsky 02, Haghighi et al. 08]. 


%Bilingual lexicon mining from non-parallel corpora has been studied for many years. \newcite{koehn2002learning} proposed to use statistical and morphological features of lexicons as a clue to construct a English-German word-level translation lexicon. \newcite{schafer2002inducing} exploit the idea that word translations tend to co-occur in time across languages, and uses this and other similarity measures to bootstrap a small seed bilingual dictionary and induce full dictionaries for low resource languages \cite{schafer2006translation}. 

%Name translation mining can be considered as a special bi-lingual lexicon mining task.  \newcite{klementiev2006weakly} used the temporal cue combined with phonetic similarity to mine name translations. \newcite{ji2009mining} proposed to use information extraction techniques to mine name translations from comparable corpora. Ji2011



%To start deciphering the Chinese BINet, we need a few seeds based on prior knowledge as a starting point. Inspired by some previous work on bi-lingual dictionary induction (e.g.,~\cite{koehn2002learning,Irvine2013}), decipherment (e.g.,~\cite{Ravi2011,Dou2012,Dou2014}) and name translation mining (e.g.,~\cite{ji2009mining,Lin2011}), we utilize some minimal linguistic resources - a bi-lingual lexicon and language-universal representations such as time/calendar date, number, website URL, currency and emoticons to decipher a small subset of Chinese nodes. For the example shown in Figure \ref{fig:walkthrough}, we can decipher some nodes in the Chinese BINet such as ``7-6'' and ``种子(seed)''.

%previous mining work also used temporal constraints, but we proposed co-burst graph... graph topological structure...; co-burst graph is also very cheap to construct 
%based on graph based on burst. richer clues. no need IE
%bilingual lexicon mining
%name translation mining. dan roth and ji both use temporal information. 
%temporal constraints for other tasks
%morph. entity resolution.
% also cite bi-lingual dictionary induction work by ccb, dan roth, etc. check the related work in my name mining papers
% proposed a co-occurrence based approach to build an information network where each node is a word type (i.e., term) and edges 
%burst information
%name mining
%deciperment
%novelty of decipherment, never applied to this kind of data before.
% first time apply decipherment to network structure
%decipherment
%In addition, there is work \cite{Ravi2011,Dou2012,Dou2014} regarding bilingual lexicon mining as a decipherment procedure.


%In this paper, we decipher a foreign language BINet and  regard the name translation as a decipherment procedure on a bursty information network. This is the first time to apply decipiherment to network structure.



% compare to the following work: we focus on information units instead of burst words, and we extend it to cross-lingual
%@inproceedings{sayyadi2009event,
%  title={Event Detection and Tracking in Social Streams},
%  author={Sayyadi, Hassan and Hurst, Matthew and Maykov, Alexey},
%  booktitle={ICWSM},
%  year={2009}
%}


% add burst detection related papers from data mining
% add in name translation mining papers
%: In cross-lingual slot filling, 59% of omission errors and 85% of spurious errors were due to MT errors on names [Ji et al. 09]. Following [Knight and Graehl 98] and [Hermjakob, Knight, and Daumé 08], we developed novel techniques to mine name translation pairs from non-parallel corpora [Ji 09; Lin et al. 11], re-rank name transliteration hypotheses based on bilingual IE [Ji et al. 09], jointly infer entity extraction and translation [Ji and Grishman 07], and do name-aware MT [Li et al. 13] based on joint bilingual name tagging [Li et al. 12a].


==> newpara.tex <==
Once the BINets are constructed and deciphered, many other powerful knowledge extraction mechanisms are enabled. For example, a natural bi-product of our approach is detecting the influential roles of each community. Moreover, we can utilize the BInets to disambiguate entities, construct their profiles and predict hidden relations simultaneously during the decipherment. For example, %nodes 9-17 demonstrate many potential values of deciphering the BINet. 
For node 9, deciphering the nickname ``小威'' into Serena Williams can greatly benefit cross-lingual entity linking. Nodes 10-11 and 12-13 also demonstrate that the potential effect on entity linking and coreference resolution. Nodes 14-15 also show that the deciphered BINets can help entity disambiguation. ``央行(Central bank)'' may refer to different entities during different burst periods. Moreover, the deciphered BINets can also improve entity extraction. 
%name entity recognition, which is demonstrated with the example of 
For example, in nodes 16-17. 翁山苏姬(Aung San Suu Kyi) is not recognized as a PERSON name by the Chinese name tagger; instead, it is separated into two words -- 翁山 and 苏姬. However, since 翁山 and 苏姬 are deciphered into the same English named entity -- Suu Kyi, we can merge them back to form the correct entity.
% 翁山苏姬 may be a named entity and it should not be splitted.

